From Variability to Stability: Advancing RecSys Benchmarking Practices

In the rapidly evolving domain of Recommender Systems (RecSys), new algorithms frequently claim state-of-the-art performance based on evaluations over a limited set of arbitrarily selected datasets. However, this approach may fail to holistically reflect their effectiveness due to the significant impact of dataset characteristics on algorithm performance. Addressing this deficiency, this paper introduces a novel benchmarking methodology to facilitate a fair and robust comparison of RecSys algorithms, thereby advancing evaluation practices. By utilizing a diverse set of $30$ open datasets, including two introduced in this work, and evaluating $11$ collaborative filtering algorithms across $9$ metrics, we critically examine the influence of dataset characteristics on algorithm performance. We further investigate the feasibility of aggregating outcomes from multiple datasets into a unified ranking. Through rigorous experimental analysis, we validate the reliability of our methodology under the variability of datasets, offering a benchmarking strategy that balances quality and computational demands. This methodology enables a fair yet effective means of evaluating RecSys algorithms, providing valuable guidance for future research endeavors.

==> content/old_content/1_old_intro.tex <==
% План по методологии: 
\section{Introduction}


% Maybe we need to add also 'an arbitrary set of datasets with various splitting and filtering strategies'? 
% Васильев Алексей: сюда же можно добавить что алгоритмы в статьях бывают не доученными и получают заниженные оценки

% Methodological papers criticized this way of benchmarking, providing evidence that current practices lead to false claims and misleading results.

% Введение
Recommender systems have become the backbone of personalizing user experiences across diverse online platforms. 
Suggesting movies on streaming services, proposing products for purchase, and curating personalized news feeds~\cite{krichene2020sampled}, RecSys are one of the core web technologies.
Their impact drives ongoing development in both academia and industry, resulting in the introduction of numerous RecSys algorithms each year~\cite{sun2023take}.

% Постановка проблемы
With this ongoing expansion, there is a growing need for tools that enable reproducible evaluation, allowing researchers to assess new methods alongside well-established baselines~\cite{sun2020we, ferrari2021troubling, hidasi2023effect}. 
While several frameworks \cite{anelli2021elliot, zhao2022recbole, sun2022daisyrec}
excel in conducting a rigorous evaluation of RecSys algorithms on a specific dataset, selecting the best-performing models across multiple problems remains challenging.
Results can vary significantly based on the dataset used, and what works well in one context may not perform as strongly in another~\cite{chin2022datasets}.
This variability often results in inconsistent conclusions from evaluation studies, highlighting the importance of comparing algorithms across datasets with various data characteristics. 
Researchers seek to identify universally effective algorithms across different recommendation tasks, while business users benefit from algorithm performance comparisons on datasets that reflect their specific industry domain or characteristics, aiding in informed decision-making. 


% Thus, determining the top-performing algorithms across diverse datasets holds value for both researchers and business users.
% Researchers may aim to determine a "silver bullet" or algorithm that performs well under different recommendation tasks, while business users can compare algorithm performance on datasets from the same industry domain or with similar characteristics, aiding in making informed decisions in a business setting.

% Taking into account diverse problems, domains, and dataset statistics, we have faced discrepancies in the evaluation results in different papers.
% This inconsistency across evaluations poses a dilemma: numerous algorithmic options exist, yet there's a lack of clarity on which one is the most reliable, which makes the methodology of existing solutions not fully complete.

% Существующие решения для бенчмарка (не используются для рексисов). Тоже постановка проблемы
% In machine learning, benchmarking of distinct approaches has been employed across various domains to gauge progress.
% They rank methods concerning different criteria and aggregate results over multiple datasets consistently.
% A pioneering approach based on critical differences~\cite{demvsar2006statistical} determines the best time series classification method~\cite{middlehurst2021hive} using more than $100$ tasks.
% Later, Bayesian tests~\cite{corani2017statistical, benavoli2014bayesian, benavoli2017time} report statistical significance for a difference in performance for the two methods.
% Performance curves~\cite{dolan2002benchmarking} consider
% how far away from the top approach w.r.t. the metric value a particular method is.
% Adopting Social-Choice Theory in ranking NLP models~\cite{rofin2022vote} introduced more formal definitions of fair ranking to the ML community.
% However, being diverse, advanced, and principled, these benchmarkings mostly ignore the existence and specificity of RecSys.

% Плавный переход
% However, the problem in the field of RecSys benchmarking is present. On the one hand, we have a variety of evaluation frameworks with plenty of models to test, but on the other hand, none of them are "complete" in terms of performance aggregation over multiple datasets. 
% Therefore, there is a need for the development of a new benchmark methodology.
% A holistic benchmarking methodology should reliably rank a set of methods based on performance using a diverse range of problems using offline evaluation.
% % In this way, we should be able to provide evidence for determining the best method on average and a single problem beforehand.

% Given specifics of RecSys~\cite{zhu2022bars,said2014comparative}, to ensure the reliability of a benchmarking system, we identify the following key foundational requirements that a ranking method should meet:

However, the challenge in the field of RecSys benchmarking lies in the absence of an accepted performance aggregation method across multiple datasets in contrast with other machine learning subdomains like time series classification~\cite{bellogin2017statistical} and NLP~\cite{rofin2022vote}.
Furthermore, there is a lack of research dedicated to comparing and contrasting different recommendation datasets, understanding their impact on the performance of RecSys algorithms, and identifying datasets with similar characteristics. 
% This research gap emphasizes the need for the development of a new benchmark methodology that can reliably rank RecSys methods based on their performance across various problems using offline evaluation, thereby overcoming the limitations of current practices and paving the way for more informed and effective algorithm selection.

In this work, we develop a comprehensive benchmark methodology that can reliably rank RecSys methods based on their performance across various problems using offline evaluation, thereby overcoming the limitations of current practices and paving the way for more informed and effective algorithm selection.
%With a predetermined significance level, 
Our approach enables us to confidently determine whether a specific top-1 model can excel universally across new problems or within particular domains defined by dataset characteristics. 
%While our primary focus is on the top-N recommendation task, it also extends to other domains.

Our contributions include:
\begin{itemize}
    \item The introduction of a benchmarking methodology tailored to the RecSys domain, featuring a clearly defined evaluation protocol and hyperparameter tuning with the swift integration of new algorithms~\footnote{To guarantee the reproducibility of our results, all code and datasets employed in our experiments are openly available in our GitHub repository. For access, please see \url{https://anonymous.4open.science/r/recsys-evaluation-of-dozens-datasets-0635}.}.
    % \item Comparison of ranking methods to identify the most suitable approach for the specific context of Recommender Systems. We stick to the basic requirements described above, considering metric values, agnosticism to poor algorithms, interpretability, and quantifying the significance of the difference in performance.
    
    \item Utilization of 30 public datasets for benchmarking, including the introduction of two new open-source datasets from distinct RecSys domains (music and e-commerce), accessible for download~\footnote{Will be available after peer-review.}.
    
    \item Comparative analysis of various aggregation methods and robustness stress tests to identify the most suitable approach for RecSys multi-dataset benchmarking.
    % using Spearman and Kendall correlations in line with the foundational requirements discussed.
    % This will emphasize ranks whose agnostic to ranking perturbations, paying attention to the statistical significance of performance differences.
    
    \item Investigation into the relationship between specific dataset characteristics and recommendation accuracy and identifying dataset clusters with similar characteristics.

    \item Identification of the top-performing algorithms from a pool of 12 frequently used baselines based on principled metrics aggregation across multiple scenarios.
    
\end{itemize}

% Our ultimate goal is to establish a universally accepted benchmark methodology that benefits both researchers and practitioners, providing a standardized environment to test new models against existing baselines. Our code and new datasets are available on GitHub at (https://github.com/XXXXXX/XXXX).

% Understanding that offline testing dramatically depends on having varied datasets, we respond to this ongoing need for data. 
% The paper introduces three new datasets from different areas that require recommendation systems: finance, song recommendations, and shopping behavior.

% This will offer a thorough assessment of a model's robustness in relation to varying dataset statistics and will provide a researcher with an advanced and comprehensive ranking methodology. 
% Employing a vast array of datasets, we carry out an offline evaluation, mirroring established research workflows, thus ensuring that our findings can be easily repurposed.

% Что делаем в проекте, какие цели преследуем
% We split the problem into two sub-problems: define a procedure that can provide a statistically significant pairwise and group-wise ranking of RecSys approaches and collect a large enough number of datasets to establish this significance for existing and forthcoming algorithms.
% The article presents a solution to both sub-problems.

==> content/old_content/2_old_related_work.tex <==
\section{Related work}

\textbf{\textit{RecSys evaluation.}} Recommender systems continue to be a dynamic research area.
Traditional techniques like Neighborhood-based models \cite{resnick1994grouplens, sarwar2001item} and Matrix Factorization~\cite{5197422} remain reliable baselines.
However, incorporating Deep Neural Networks has notably advanced RecSys, significantly enriching the domain~\cite{zhang2019deep}. 
This variety leads to the development of open-source libraries and tools to address diverse application needs. 
Among the noteworthy ones,  DeepRec~\cite{zhang2019deeprec}, Implicit~\cite{Implicit}, LightFM~\cite{Kula15}, NeuRec~\cite{NeuRec}, RecBole~\cite{zhao2021recbole}, RecPack~\cite{RecPack2022} and Replay~\cite{replay-rec} offer realizations of popular recommendation algorithms. 

Offline evaluation remains essential in RecSys research as it provides a reliable and cost-effective approach to assess algorithm performance. 
It is particularly suitable for researchers who are developing new models.
% When implementing AI solutions in real-world industry scenarios, offline evaluation helps to reduce the pool of candidate algorithms to a manageable number that seems promising based on the offline metrics~\cite{canamares2020target}.
% After this preliminary assessment, live testing methods, such as human expert reviews and A/B testing, are typically employed to validate the performance of the shortlisted algorithms in actual user environments~\cite{kouki2020lab}.
An emerging trend in the field is rigorous and reproducible evaluation methodologies.
Notable studies such as Elliot~\cite{anelli2021elliot}, Recbole~\cite{zhao2022recbole}, and DaisyRec~\cite{sun2022daisyrec} introduced comprehensive evaluation frameworks in both reproducing and benchmarking recommendation models. These frameworks offer a rich array of options for pre-filtering, data splitting, evaluation metrics, and hyperparameter tuning across a broad spectrum of popular recommender models.  
Notably, Elliot uniquely provides statistical tests for robustly analyzing the final results, adding a layer to the evaluation process.

\textbf{\textit{RecSys datasets.}} Dozens of public datasets from diverse domains are available for constructing and evaluating recommender systems. The research~\cite{zhao2022revisiting} shows that most studies utilize an average of 2.9 datasets, with dataset selection and preprocessing affecting evaluation outcomes significantly.
% examined dataset selection and preprocessing trends, identifying that recent studies typically utilize an average of 2.9 public datasets. The research 
% emphasizes the critical need for diverse dataset selection and 
% investigates the impact of different filtering approaches on performance evaluation metrics, discovering that these strategies can significantly change data characteristics, thus leading to different performance ranking results.
% This underscores the recommendation for using varied datasets to ensure broad evaluation coverage and cautions against the potential biases introduced by specific data filtering techniques. 
Different data filtering techniques can change data characteristics, leading to varied performance rankings.
Deldjoo et al.~\cite{deldjoo2020dataset, deldjoo2021explaining}
investigated how data properties impact recommendation accuracy, fairness, and vulnerability to shilling attacks, highlighting the importance of data understanding in enhancing system performance.
% investigate the impact of data characteristics on recommender systems using regression-based models. Their initial work explores various data characteristics and their influence on recommendation accuracy and fairness, while a subsequent study delves into shilling attacks against collaborative filtering models and how different user-item matrix properties affect susceptibility. Both studies underscore the significance of understanding and handling data characteristics to improve recommender system performance.
The paper~\cite{chin2022datasets} emphasized the crucial role of dataset diversity in RecSys algorithm evaluations, showing that dataset choice significantly affects evaluation conclusions. These findings collectively underscore the need for considering dataset variability in future research to enhance the reliability of recommender system evaluations.
% provides a detailed examination of dataset selection in the evaluation of RecSys algorithms, a crucial yet often overlooked aspect. It analyzes recent literature to understand how datasets are utilized and compares the characteristics of these datasets. Through empirical studies, the paper demonstrates that the choice of datasets can influence the conclusions drawn from evaluations. It advocates for using datasets with diverse characteristics to enhance the robustness of evaluations, highlighting the limitations of relying on common benchmark datasets. 
% The findings underscore the importance of considering dataset variability in future research to improve the reliability of recommender system evaluations.

\textbf{\textit{Aggregating methods.}} When introducing a novel machine learning approach, it is important to rigorously compare its performance against existing methods across a comprehensive set of relevant tasks to determine its standing relative to the current state-of-the-art. 
% In benchmarking, the methods under comparison are referred to as "comparates".
% When a set of \textit{$m$} comparates is evaluated across \textit{$d$} tasks, it generates task-specific outcomes (e.g., \textit{nDCG@10} in RecSys) for each comparate on each task, leading to a total of \textit{m × d} outcomes. 
However, drawing conclusions about the superior algorithm based on the outcomes from multi-dataset benchmarks  can be challenging.
Various techniques have been developed to yield concise summaries to address this challenge.
% The most straightforward approach is to employ mean aggregation, which assumes that all task metrics are homogeneous~\cite{colombo2022infolm}. 
% In cases where metrics are heterogeneous, 
% as is often the scenario in RecSys or NLP, the mean aggregation disregards the relative ordering of tasks.
% It relies solely on absolute score differences, treating tasks of varying complexities and from different domains equally.
% this approach leads to biased evaluations and subjective outcomes~\cite{niessl2022over}.

One basic method involves mean aggregation, assuming uniformity across task metrics~\cite{colombo2022infolm}. However, this can lead to biased evaluations when metrics vary significantly~\cite{niessl2022over}. 
The Dolan-Moré performance profiles, initially developed for optimization algorithm benchmarks~\cite{dolan2002benchmarking}, has gained traction for evaluating machine learning algorithm efficacy across diverse problems~\cite{belyaev2016gtapprox}.
Unlike mean aggregation, Dolan-Moré curves consider the distribution of performance values, offering insight into how frequently and significantly one algorithm excels. 
% While these curves may not directly evaluate the quality of one method compared to another, they still serve as a valid option for benchmarking to identify the algorithm that performs best~\cite{gould2016note}. 
Similarly, the Critical Difference diagram (CD diagram)~\cite{demvsar2006statistical} is frequently used to compare algorithms across multiple tasks.
This method of presenting results has become broadly ~\cite{middlehurst2021hive}.
% In the domain of time series classification, its use is now prevalent. 
The CD diagram provides both groupwise and pairwise comparisons. 
Groupwise comparisons are achieved by ordering all comparates based on the mean rank of relative performance on each task. 
Pairwise comparisons are based on a critical difference in this mean rank or, in newer version~\cite{benavoli2016should}, the Wilcoxon signed-rank test~\cite{wilcoxon1992individual} with multiple test corrections. 

% A subsequent work~\cite{benavoli2017time} concentrates on improving the procedure for establishing whether or not a pairwise difference in accuracy is statistically significant, adopting Bayesian approaches, for instance, hierarchical models~\cite{corani2017statistical}. 
% However, the use of the CD diagram remains unchanged mainly since 2006~\cite{demvsar2006statistical}, despite well-known
% shortcomings relating to the underlying statistical methods. 
% For example, the method is open to cheating, potentially distorting the impression conveyed by the results %~\cite{ismail2023approach}
% by including a maliciously designed method in a group comparison.

VOTE'N'RANK~\cite{rofin2022vote} is a framework proposed for ranking systems in multitask benchmarks rooted in the principles of social choice theory.
% The primary motivation for this approach is the perceived limitation of the current benchmarking methods, which often rely on mean scores across tasks.
% Such methods might give a misleading sense of progress in machine learning research.
The framework employs scoring and majority-relation-based rules, such as Plurality, Dowdall, Borda, Copeland, and Minimax, to ensure a more comprehensive evaluation.

% \textbf{\textit{Research gap.}} 
\textbf{\textit{Benchmarking}} is a fundamental practice in computer science and machine learning, crucial for measuring progress through datasets, metrics, and aggregation methodologies to evaluate system performance. These benchmarks are crucial for comparing new algorithms with established ones to identify the most effective models for practical use.
% common in computer science and machine learning to measure progress. 
% In Machine Learning, benchmarks typically encompass datasets accompanied by one or more metrics and an aggregation methodology to evaluate the performance of a system.
% These evaluations play an instrumental role in comparing emerging algorithms with established ones, thereby identifying the most productive models for real-world applications.

% Various domains rely on performance benchmarks to assess and drive advancements.
% For instance, 
Performance benchmarks are essential across various fields. For example, 
the ILSVRC (ImageNet Large Scale Visual Recognition Challenge)~\cite{russakovsky2015imagenet} benchmarks object classification and detection with extensive image datasets and unique metrics for each task. 
In natural language processing (NLP), GLUE~\cite{wang2018glue} and its derivatives~\cite{wang2019superglue} benchmark models across diverse tasks, ranking them based on mean score values.
One example in the AutoML domain is AMLB~\cite{gijsbers2022amlb}, which emphasizes multitask evaluation via mean ranking.
% AMLB~\cite{gijsbers2022amlb} is a recent benchmark in the AutoML domain, employing a multitask approach, using mean rank as its primary ranking method.

The research~\cite{anelli2022top} offers an in-depth and reproducible evaluation of ten collaborative filtering algorithms, employing a Borda count ranking method to aggregate accuracy results from various datasets and metrics. The study emphasizes that, although this method provides valuable insights, it necessitates careful interpretation due to biases favoring algorithms that perform well in correlated metrics.

\begin{figure*}[!th]
    \centering
    \includegraphics[width=0.98\textwidth]{images/Benchmark_draft.pdf}
    \caption{The proposed benchmarking for the ranking of algorithms. Our main innovations are the curated list of datasets that enable the option of comparison of pairs of models and aggregation strategies that provide principled ranking of approaches w.r.t. various criteria.}
    \label{fig:pipeline_scheme}
\end{figure*}
~\cite{anelli2022top}
To the best of our knowledge, BARS~\cite{zhu2022bars} is the most advanced benchmarking initiative focused on RecSys. 
% tasks related to Click-through rate prediction and Candidate Item Matching. 
Although BARS strives to establish an open benchmark with standardized evaluation protocols, it presents certain limitations.
For instance, it restricts itself to only three datasets dedicated to the singular challenge of top-N recommendation, maintaining discrete leaderboards for each dataset.
Such an approach, devoid of a multi-dataset scoring mechanism, inhibits discerning truly adaptive and universal models — covering this gap might offer significant insights for researchers.

% To create a robust benchmark within RecSys, one should use a diverse set of datasets and models and a rigorous evaluation pipeline. 
% Finding and testing the best ranking methods suitable for various scenarios is also essential.
% Our goal is to closely examine these methods in the RecSys setting and define the most valuable ones to extend well-established evaluation methodology steps.
